Paraclassical Logics with Two Negations

We study three paraclassical propositional logics with two negations, CLoaN, CLouN, and CLauN, obtained by pairwise combining the one-negation systems CLuN, CLaN, and CLoN. CLuN's negation is glut-tolerant and paraconsistent, CLaN's negationis gap-tolerant and paracomplete, and CLoN's negation is both paraconsistent and paracomplete. We provide sound and complete two-valued non-deterministic semantics for each of the two-negations systems. We then focus on CLauN, the system containing the primitive dual pair of CLaN and CLuN negations. In this setting, we show deductive relationships between different negations expressible in CLauN; we show two diferent ways to recapture classical logic by means of translations, locally and globally; and we show a duality results for the multiple conclusion consequence relation of the logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{119}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.10}{10.4204/EPTCS.455.10}}

